Deep Active Surface Models

Active Surface Models have a long history of being useful to model complex 3D surfaces but only Active Contours have been used in conjunction with deep networks, and then only to produce the data term as well as meta-parameter maps controlling them. In this paper, we advocate a much tighter integration. We introduce layers that implement them that can be integrated seamlessly into Graph Convolutional Networks to enforce sophisticated smoothness priors at an acceptable computational cost. We will show that the resulting Deep Active Surface Models outperform equivalent architectures that use traditional regularization loss terms to impose smoothness priors for 3D surface reconstruction from 2D images and for 3D volume segmentation.

==> results/shapenet.tex <==
\begin{table*}[!htbp]
	\label{table:shapenet_results_diff_lambda}
	\begin{tabular}{l|l|cccc}
		\hline
	$\lambda$						&  							& Chf. ($\downarrow$)& Normal &  $F^{0.1}$  &  $F^{0.5}$\\ \Xhline{3\arrayrulewidth}
	\multirow{2}{*}{1.0}   	& \meshrcnn{}  &     a    &                a & a       &    a   \\
									        & \dasm{}			 &         &        			&              &                \\ \hline
 
	\multirow{2}{*}{0.6}   	& \meshrcnn{} &   0.212     			  &        0.681                      &     30.6    &   \textbf{91.4}\\
												& \dasm{} 			&   \textbf{0.206}      &       \textbf{0.693 }		&    \textbf{31.4 }    &      \textbf{91.4 }         \\ \hline

	\multirow{2}{*}{0.2}   	& \meshrcnn{} &   0.189      			  &        0.691                      &     32.8    &   \textbf{92.6}\\
									        & \dasm{} 			&   \textbf{0.183}      &       \textbf{0.727 }		&    \textbf{33.5 }    &      {92.5 }         \\ \hline
	 
	\multirow{2}{*}{0.0}   	& \meshrcnn{} &   \textbf{0.144}      &        0.713              &      \textbf{35.8}     &    \textbf{94.2} \\
									         & \dasm{} 			&    0.167                     &        \textbf{0.718} 				&      34.3       &         93.9          \\ \hline
	\end{tabular}
\end{table*}

%\begin{table*}[!htbp]
%	\begin{tabular}{l|l|lllllll}
%		\hline
%		$\lambda$	&  & Chf. ($\downarrow$)& Normal & $F^{0.1}$ & $F^{0.3}$ & $F^{0.5}$ \\ \Xhline{3\arrayrulewidth}
%		\multirow{2}{*}{1.0}   	& \meshrcnn{} &     a    &     a   &       a  &       a & a              \\
%		& \dasm{} &         &        &         &            &           \\ \hline
%		
%		\multirow{2}{*}{0.6}   	& \meshrcnn{} &         &        &         &          &           \\
%		& \dasm{} &         &        &         &          &    \\ \hline		 
%		
%		\multirow{2}{*}{0.2}   	& \meshrcnn{} &         &        &         &       &              \\
%		& \dasm{} &         &        &         &          &        \\ \hline
%		
%		\multirow{2}{*}{0.0}   	& \meshrcnn{} &         &        &         &      &               \\
%		& \dasm{} &         &        &         &         &         &        &  \\ \hline
%	\end{tabular}
%\end{table*}

%0.182642  | 0.726924 | 33.5322   | 81.0172   | 92.5215   |

==> tables/abolation.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[]
	\label{abolation}
	\begin{tabular}{|l|c|}
		\hline
		~                                                  & Chamfer Dist. $\times 10^{-3}$ \\ \hline
		\voxm{}                                                 & 4.7 $\pm$ 0.8     \\ \hline
		\voxm{} - bottom up                                     & 4.3 $\pm$ 1.3     \\ \hline
		+ Voxel decoder                                            & 2.8 $\pm$ 0.9     \\ \hline
		+ Voxel decoder + $\mathcal{L}_{ce}$                       & 2.4 $\pm$ 0.4     \\ \hline
		+ Voxel decoder + $\mathcal{L}_{ce}$ + $\mathcal{L}_{mse}$ & 2.4 $\pm$ 0.3     \\ \hline
		+ iterative refinement & 2.3 $\pm$ 0.3     \\ \hline
	\end{tabular}
	\caption{Ablation study results summary for the surface decoder on liver datasets}
\end{table}

==> tables/document.tex <==
\begin{table}[]
\begin{tabular}{lll}
Tr. set size & U-Net & \vmnet{} \\
10           & 76.3 \pm 3.6 & 79.2 \pm 2.0   \\
50           & 77.8  \pm 0.1& 79.3 \pm 0.4 \\
90           & 79.5 \pm 0.2 & 79.9 \pm 0.5  \\
130          & 80.2 \pm 0.2 & 81.3   \pm 0.3
\end{tabular}
\end{table}

==> tables/main_results.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table*}[htbp]
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}}             & \multicolumn{2}{c|}{Liver}    & \multicolumn{2}{c|}{Hippocampus}           \\ \cline{3-6} 
\multicolumn{2}{|l|}{}                                     & \begin{tabular}[c]{@{}l@{}}Chamfer Dist. $\times 10^{-3}$ \end{tabular} & IoU & \begin{tabular}[c]{@{}l@{}}Chamfer Dist. $\times  10^{-3}$  \end{tabular} & IoU \\ \hline
\multicolumn{2}{|l|}{\vnet{}} 												  &   -     &  		67.4 $\pm$ 2.3				   &  -  &  59.4 $\pm$ 2.2   \\ \hline
\multicolumn{2}{|l|}{\unet{}}											      &   -     &  76.3 $\pm$ 3.6  &  -  & 70.9 $\pm$ 3.5    \\ \hline
\multicolumn{2}{|l|}{\voxm{}} 					&   4.7 $\pm${0.8}     &  -   & 2.4 $\pm$ 0.3  &  -    \\ \hline\hline
\multicolumn{2}{|l|}{\vmnet{}}                    			&  \textbf{ 2.3 }$\pm$  0.3   &  \textbf{79.2} $\pm$ 2.0 	& \textbf{1.9} $\pm$  0.1 &  \textbf{73.5 }$\pm$ 0.7   \\ \hline
%\multicolumn{1}{|c|}{\multirow{2}{*}{Ours}} & Voxel branch  &   -     &   \textbf{79.2} $\pm$ 2.0 &  -  &  \textbf{73.5 }$\pm$ 0.7 \\ \cline{2-6} 
%\multicolumn{1}{|c|}{}                      			& Mesh branch  &  \textbf{ 2.5 }$\pm$  1.0   &  67.9 $\pm$  2.6	& \textbf{1.9} $\pm$  0.1 &  65.2 $\pm$ 0.6    \\ \hline
\end{tabular}
\caption{{\bf Comparative results on our two datasets.} \vmnet{} outperforms the baselines on both.}
\label{table:main_results}
\end{table*}


% 400 : 2
% 430 : 2
% 410 : 1

==> tables/results_32.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
	\centering
\caption{Comparative results at resolution $32 \times 32 \times 32$. Cmf. refers to Chamfer distance and IoU is the intersection of union.}
\label{table:liver_at_32_resolution}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}}                    & \multicolumn{2}{c|}{Liver}                                      & \multicolumn{2}{c|}{Hippocampus}                                \\ \cline{3-6} 
\multicolumn{2}{|l|}{}                                     & \begin{tabular}[c]{@{}l@{}}Cmf.\end{tabular} & IoU & \begin{tabular}[c]{@{}l@{}}Cmf.\end{tabular} & IoU \\ \hline
\multicolumn{2}{|l|}{V-Net}  &   &   &   &     \\ \hline
\multicolumn{2}{|l|}{U-Net}  &- & 58.4  &   &     \\ \hline
\multicolumn{2}{|l|}{Pix2Mesh (adopted)}  &  &  &   &     \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Ours}} & Voxel branch & -  & 56.9 &   &     \\ \cline{2-6} 
\multicolumn{1}{|c|}{}                      & Mesh branch  & -  &\textbf{67.8}&     &     \\ \hline
\end{tabular}
\end{table*}

==> tables/results_64.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Comparative results on the two datasets. Cmf. refers to Chamfer distance and IoU is the intersection of union.}
\label{table:main_results}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{}}                    & \multicolumn{2}{c|}{Liver}                                      & \multicolumn{2}{c|}{Hippocampus}                                \\ \cline{3-6} 
\multicolumn{2}{|l|}{}                                     & \begin{tabular}[c]{@{}l@{}}Chamfer Dist. $\times 10^{-3}$ \end{tabular} & IoU & \begin{tabular}[c]{@{}l@{}}Chamfer Dist. $\times  10^{-3}$  \end{tabular} & IoU \\ \hline
\multicolumn{2}{|l|}{V-Net} 												  &   -     &  		67.4 $\pm$ 2.3				   &  -  &  59.4 $\pm$ 2.2   \\ \hline
\multicolumn{2}{|l|}{U-Net} 											      &   -     &  76.3 $\pm$ 3.6  &  -  & 70.9 $\pm$ 3.5    \\ \hline
\multicolumn{2}{|l|}{Pix2Mesh (adopted)}   							 &   4.7 $\pm${0.8}     &    & 2.4 $\pm$ 0.3  &     \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Ours}} & Voxel branch  &   -     &   \textbf{79.2} $\pm$ 2.0 &  -  &  \textbf{73.5 }$\pm$ 0.7 \\ \cline{2-6} 

\multicolumn{1}{|c|}{}                      			& Mesh branch  &  \textbf{ 2.5 }$\pm$  1.0   &  67.9 $\pm$  2.6	& \textbf{1.9} $\pm$  0.1 &  65.2 $\pm$ 0.6    \\ \hline
\end{tabular}
\end{table*}

==> tables/tr_size.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[]
	\centering
	\begin{tabular}{|l|l|l|}
		\hline
Tr. set size & \unet{} & \vmnet{} \\ \hline
10           & 70.9 $\pm$ 3.5 & \textbf{73.5} $\pm$ 0.7   \\ \hline
50           & 77.8  $\pm$ 0.1& \textbf{79.3} $\pm$ 0.4 \\ \hline
90           & 79.5 $\pm$ 0.2 & \textbf{79.9} $ \pm $  0.5  \\ \hline
130          & 80.2 $\pm$ 0.2 & \textbf{81.3} $ \pm $ 0.3 \\  \hline
	\end{tabular}
	\caption{Increasing the size of the training set.}
\label{tab:tr_size}
\end{table}

==> tex/3_method_2.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US
 
\section{Method} 
\label{sec:method}

We first introduce the general formulation of Active Surface Models (ASMs) and then show how we can apply it to meshes whose vertices can be of arbitrary degree. Finally, we discuss the integration of ASMs and mesh-deforming Graph-Convolutional Neural Networks (GCNNs), which produces our Deep Active Surface Models (DASMs). 

\subsection{Active Surface Model (ASM)}
\label{sec:asm}

An ASM consists of a surface $\mS(\Phi)$ whose shape is controlled by a vector of parameters $\Phi$ and can be deformed to minimize an objective function $E(\Phi)$, often referred to as an {\it energy}. We first introduce a continuous formulation and then its discretization, which is the one used in practice. 

\parag{Continuous Formulation.} $\mS$ is represented by the mapping from $\mathbb{R}^2$ to  $\mathbb{R}^3$
%
\begin{equation}\label{eq:surface}
 v: (s,r;\Phi)  \mapsto (v_x(s,r;\Phi), v_y(s,r;\Phi), v_z(s,r;\Phi)) \; ,
\end{equation}
%
where $(s,r) \in \Omega = [0, 1] \times [0, 1]$. Fig.~\ref{fig:surface_derivative} depicts this mapping and its derivatives. $\Phi$ is typically taken to be 
\begin{align}\label{eq:minimize1}
   \Phi^*    &= \argmin_{\Phi} E(\Phi) \; , \\ 
    E(\Phi) & = E_{\rm dat} (\Phi) + E_{\rm def} (\Phi) \nonumber ,
\end{align}
%
where $E_{\rm dat}$ is a data term that measures how well the surface matches the images and $E_{\rm def}$ is a deformation energy that is smallest when the surface is smooth. $E_{\rm def}$ is often written as
%
\begin{align}\label{eq:deformation1}
E_{\rm def} = & \int_{\Omega} w_{10} \left\lVert \frac{\partial v}{\partial s} \right\lVert^2 + w_{01} \left\lVert \frac{\partial v}{\partial r} \right\lVert^2
+ 2w_{11} \left\lVert \frac{\partial^2 v}{\partial s \partial r} \right\lVert^2 \nonumber \\
& + w_{20} \left\lVert \frac{\partial^2 v}{\partial s^2} \right\lVert^2 + w_{02} \left\lVert \frac{\partial^2 v}{\partial r^2} \right\lVert^2 dr ds\; .
\end{align}
%

\parag{Discrete Formulation.}

When $\mS(\Phi)$ is discretized and represented by a triangulated mesh $\mM(\Phi)$, $\Phi$ becomes the $3N$-vector built by concatenating the 3D coordinates of its $N$ vertices. Using the finite-difference approximation described below, the deformation energy can be rewritten as
%
\begin{align}\label{eq:deformation2} 
E_{\rm def} = \frac{1}{2} \Phi^t \bA \Phi \; ,
\end{align}
%
where $\bA$ is very sparse square matrix. 
%
For $\Phi^*$ to minimize $E(\Phi)$, we must therefore have
\begin{align}\label{eq:minimize2}
 0 & =   \nabla E_{\rm dat} (\Phi^*) + \nabla E_{\rm def} (\Phi^*) \nonumber , \\
    & =   F(\Phi^*) + \bA \Phi^* \; ,
\end{align}
%
where $F=\nabla E_{\rm dat}$. Because $\bA$ is usually non-invertible, given an initial value $\Phi^0$, a solution to this equation is usually found by iteratively solving 
%
\begin{align}
0 & = F(\Phi^{t-1}) + \bA \Phi^t + \alpha ( \Phi^t - \Phi^{t-1} ) \; , \nonumber  \\
   & \Rightarrow  (\bA + \alpha \bI) \Phi^t =  \alpha  \Phi^{t-1} -  F(\Phi^{t-1}) \; , \label{eq:viscosity}
\end{align}
%
where $\bI$ is the identity matrix. When the process stabilizes, $\Phi^{t} = \Phi^{t-1}$ and is a solution of Eq.~\ref{eq:minimize2}. The strength of this semi-implicit optimization scheme is that it propagates smoothness constraints much faster than traditional gradient descent and at a low computational cost because $\bA$ is sparse, which means that the linear system of Eq.~\ref{eq:viscosity} can be solved efficiently. In this scheme $\alpha$ plays the role of the inverse of a step size: When $\alpha$ is large enough for the Froebinius norm of $\alpha \bI$ to be much larger than that of $\bA$, the optimizer performs a steepest gradient step with learning rate $\frac{1}{\alpha}$ at each iteration. Conversely, when $\alpha$ is small, $\bA$ dominates and much larger steps can be taken.

\PUW{Isn't the optimizer always taking the steepest step that reduce the total energy? isn't $alpha$ determining the relative weights on data term and deformation terms?}. \PF{Check what happens when $\alpha$ goes to infinity.}
\PF{No. It does not! Normally, you solve the linear system WITHOUT explicitly inverting the matrix.}
\PUW{we don't take the inverse, instead we approximate it using the matrix version of Taylor expansion for 1/(1+x)}

In the original deformable contour models~\cite{Kass88},  the matrix $\bA + \alpha \bI$ was never inverted. Instead Eq.~\ref{eq:viscosity} was solved by LU decomposition. \PF{Say why doing so is impractical in our case.} Instead, we approximate  $\bA + \alpha \bI$ using the Neumann series
%
\begin{align}\label{eq:inverse} 
& (\bA + \alpha \bI) ^{-1} \approx \sum_{n=0}^{K} (-1)^n \left(\frac{1}{\alpha}\right)^{n+1}A^n \; .
\end{align} 
% 
In practice, we use $K=4$, which gives us a sufficiently accurate approximation.

%\puw{
%Solving Eq.~\ref{eq:viscosity} requires inverting the matrix $ (\bA + \alpha \bI) $.  Since its a computationally expensive operation, we expand it using the Neumann series and approximate it by taking only the sum of first $K$ terms;
%\begin{align}\label{eq:inverse} 
%& (\bA + \alpha \bI) ^{-1} \approx \sum_{n=0}^{K} (-1)^n \left(\frac{1}{\alpha}\right)^{n+1}A^n
%\end{align} 
%For our experiments, we observe a value of $K=4$ gives sufficiently accurate approximation.
%}

\parag{Computing the Regularization Matrix  $\bA$.}

In most traditional ASMs, the meshes are either square or hexagonal and regular, which makes the computation of the derivatives of the mesh vertices possible using finite-differences and, hence, the regularization matrix $\bA$ of Eq.~\ref{eq:minimize2} easy to populate. When the mesh is triangular and irregular, vertices can have any number of neighbors and the computation becomes more complex. 

Nevertheless the derivatives from order to 2 to order 4 can still be expressed as finite differences of weighted sums of vertex coordinates where the weights are barycentric coordinates of small perturbations of the original vertices.  \PF{Why order 4?} This is illustrated by Fig.~\ref{fig:finite_differences} and explained in more details in appendix.

\input{fig/surface}

%Traditionally, ASM has been limited to regular square (degree 4) \cite{x} or hexagonal (degree 6) \cite{x} meshes. This is because, when writing finite difference equations, $v(s + k_1\delta, r + k_2\delta)$ where $ (k_1, k_2) \in  \{-1, 0, 1\}  \times \{-1, 0, 1\} \cup \{-2, 2\} \times \{0\} \cup \{0\} \times \{-2, 2\} $ terms corresponds to neighboring vertices in the mesh. When dealing with irregular meshes, we have vertices with degree other than 4 or 6. In such situations, $v(s + k_1\delta, r + k_2\delta), (k_1, k_2)$ does not corresponds to neighboring vertices in the mesh. To circumvent the limitation, we define $v(s + k_1\delta, r + k_2\delta), (k_1, k_2)$ as a linear combinations of neighboring vertices. 

%\begin{equation}\label{eq:surface}
%v(s + k_1\delta, r + k_2\delta) = \sum_{v \in \Gamma } w_v * v
%\end{equation}
%where $\Gamma$ is the set of three vertices that enclose$v(s + k_1\delta, r + k_2\delta) $. This always include the center vertex $v(s,r)$ and two more vertices from 1-ring neighborhood of $v(s,r)$. $w_v$ are the barycentric coordinates of $v(s + k_1\delta, r + k_2\delta)$ w.r.t vertices in $\Gamma$. The relative position of $v(s + k_1\delta, r + k_2\delta)$ terms w.r.t $\Gamma$ change for different degrees as shown in Fig~\ref{fig:finite_differences}.
 
\subsection{Deep Active Surface Model (DASM)}

The update equation is a typical mesh-deforming graph-convolutional neural network (GCNN) that plays the same role as that of Eq.~\ref{eq:viscosity} is
%
\begin{equation}
\Phi^t =  \Phi^{t-1} -  \frac{1}{\alpha} F(\Phi^{t-1},\bX^{t-1}) \; ,
\label{eq:grad}
\end{equation}
where $F$ denotes the gradient of the loss function calculated using the feature vector $\bX^{t-1}$ the GCNN produces given the mesh parameters $\Phi^{t-1}$. \PF{Do we need to explicitly introduce $\bX$?}. In the case of our deep active surface models, it becomes
\begin{equation}
(\bA + \alpha \bI) \Phi^t =  \alpha  \Phi^{t-1} -  F(\Phi^{t-1},\bX^{t-1}) \; ,
\label{eq:impl}
\end{equation}
as in Eq.~\ref{eq:viscosity}. In Eq.~\ref{eq:grad}, the loss function typically includes a regularization term to to keep the mesh smooth, whereas in Eq.~\ref{eq:impl} it does not because our semi-implicit scheme enforces smoothness by solving the linear equation. 

%With the exception of the term  $ (\bA + \alpha \bI) $, Eq.~\ref{eq:viscosity} resembles the standard vertex update step used in mesh-deforming graph-convolutional neural networks (GCNNs). As discussed above, for large values of $\alpha$ it is almost equivalent:  The function $F(\Phi^{t-1})$  is the output from the GC layer and would be written as $F(\Phi^{t-1}, X^{t-1})$ where $X^{t-1}$ is the set of features associated with vertices in $\Phi^{t-1}$. In a GCNN, multiple GC layers are used to deform a mesh step-by-step. This resembles the iterative surface evolution indicated by the time variable $t$. The additional term ASM introduce is $ (\bA + \alpha \bI) $. Since this is integrated with a matrix multiplication, it does not affect the differentiability of the vertex update step. 


\paragraph{Uniform vs Adaptive DASMs}

Eq.~\ref{eq:impl} forms the basis of the simplest version of our of our DASMs, which we will refer to as Uniform-DASMs because the same amount of smoothing is applied across the whole mesh. This is may result in under- or over-smoothing because some parts of the objects are typically smoother than others. 

To account for this, we also introduce Adaptive DASMs that are designed to smooth only where such smoothing is required. To this end, we replace the $\alpha \bI$ term of Eq.~\ref{eq:impl} by a diagonal matrix $\Lambda$, as in \cite{X}. \PF{$\Lambda$ is produced by another network branch?}




%-------
% OLD 
%-------



%Let $F = \nabla E_{\rm dat}$ be the gradient of $E_{\rm dat}$ with respect to $\Phi$. A necessary condition for $\Phi$ to be a local minimum of the total energy $E$ of Eq.~\ref{eq:minimize} is that it satisfies the Euler-Lagrange equation \cite{X}
%
%\begin{align}
%0 &= \nabla E_{\rm def} (\Phi) + F \\ 
%   &= F + \frac{\partial}{\partial s} \Bigg ( w_{10}  \frac{\partial v}{\partial s} \Bigg ) +  \frac{\partial}{\partial r} \Bigg ( w_{01}  \frac{\partial v}{\partial r} \Bigg )\\
%    &+ 2 \frac{\partial ^2}{\partial s \partial r} \Bigg ( w_{11}  \frac{\partial^2 v}{\partial s \partial r}\Bigg )
%+ \frac{\partial}{\partial^2 s} \Bigg ( w_{20}  \frac{\partial^2 v}{\partial s^2} \Bigg )
%+ \frac{\partial}{\partial^2 r} \Bigg ( w_{02}  \frac{\partial^2 v}{\partial r^2} \Bigg )
%\end{align}
%




%
%The associated energy
%\begin{multline}\label{eq:enery}
%E(v) = \int_{\Omega} w_{10} \left\lVert \frac{\partial v}{\partial s} \right\lVert^2 + w_{01} \left\lVert \frac{\partial v}{\partial r} \right\lVert^2
%+ 2w_{11} \left\lVert \frac{\partial^2 v}{\partial s \partial r} \right\lVert^2 \\
%+ w_{20} \left\lVert \frac{\partial^2 v}{\partial s^2} \right\lVert^2
%+ w_{02} \left\lVert \frac{\partial^2 v}{\partial r^2} \right\lVert^2 + P(v(s,r)) \partial r \partial s
%\end{multline} 
%
%
%where the term $P(v(s,r))$ which is referred to as the `external energy' quantify how well the surface $\mS$ matches the target shape while the rest of the terms which are referred to as the 'internal energy'  are the surface derivatives as shown in Fig. and introduces priors on surface elasticity, smoothness and the resistance to twist.
%
%The objective is to minimize the total energy $\bE$. Even though there is no general rule regarding a global minimum, any local minima satisfies the associated Euler-Lagrange equation \cite{x}:
%\begin{multline}\label{eq:euler}
% - \frac{\partial}{\partial s} \Bigg ( w_{10}  \frac{\partial v}{\partial s} \Bigg )
%- \frac{\partial}{\partial r} \Bigg ( w_{01}  \frac{\partial v}{\partial r} \Bigg )\\
%+ 2 \frac{\partial ^2}{\partial s \partial r} \Bigg ( w_{11}  \frac{\partial^2 v}{\partial s \partial r}\Bigg )
%+ \frac{\partial}{\partial^2 s} \Bigg ( w_{20}  \frac{\partial^2 v}{\partial s^2} \Bigg )
%+ \frac{\partial}{\partial^2 r} \Bigg ( w_{02}  \frac{\partial^2 v}{\partial r^2} \Bigg ) \\
%= F(v) 
%\end{multline} 
%subject to boundary conditions. Here $F(v) = \nabla P(v)$. To find the curve that satisfy \ref{eq:euler}, curve evolution is used by introducing a time $t$ parameter to \ref{eq:euler}
%\begin{equation}\label{eq:evolution}
%\frac{\partial v(t)}{\partial t} + L(v(t)) = F(v(t)) 
%\end{equation}
%Solving \ref{eq:evolution}, requires specifying an initial surface. Earlier approaches \cite{} used a manual initialization where as \cite{} used another model to predict the initial curve. To make sure the reached local minima corresponds to the desired curve, these approaches make sure the initialization is closer to the target shape.
 
%\subsection{Finite Difference Solution}
%\label{sec:fd_solution}
%Finding a numerical solution to the equation \ref{eq:euler} first require the discretization of the surface.  For this we use a discrete mesh $\bM = (\bV, \bF)$ where $\bV = \{v_i| v_i \in \real^3\}_{i=1}^N$ is the set of vertices and $\bF = \{f_i| v_i \in \real^3\}_{i=1}^M$ is the set of faces. $N, M$ are the number of vertices and faces, respectively.  Then, the finite difference (FD) method is to the equation {eq:evolution}:  
%\begin{equation}\label{eq:evolution}
%\frac{V^t - V^{t-1}}{\tau} + AV^t = F(V^t) 
%\end{equation}
%Here, $t$ is the time step,  $A = -w_{10}A_{10} - w_{01}A_{01} + 2w_{22}A_{10}  + w_{20}A_{20}  + w_{02}A_{02} $ and $AV^t$ is the sum of all weighted gradients.
%
%Each $A_{.}$ is a sparse matrix in which non zero elements at $i^{th}$ row corresponds the coefficients from the FD approximation of the derivative at $i^{th}$ vertex (see Appendix \ref{x}).   With 2D Active Contour models, finding $A_{.}$ is straight forward since the curve is a ordered set of points and adjacent contour points that appear in FD equations directly corresponds to adjacent points in the ordered set. Extending the same idea in to 3D Active Surface models, \cite{} use regular square or hexagonal meshes. But to model complex shapes and to be compatible with recent mesh-deforming work, we need to find  FD approximation for irregular meshes.
%
%\subsection{Relationship with Mesh Deforming Neural Networks}
%\label{sec:ac_mesh_conv_link}
%
%
%
%The energy of the curve $\bE$ is 
%\subsection{Mesh Subdivision}

==> tex/6_future_work.tex <==
\section{Future Work}
\puw{
As future work we plan on further improving adaptive version of DASM. At the moment adaptive DASM rely on a metric that predict anomalies based on surface gradients. This is not ideal since having an elongated facet does not necessarily mean it is an anomaly. Therefore, a learning based approach to predict this metric is preferred. This has been done when integrating Active Contour models with CNNs. There, they use CNN to produce maps that decide the amount of smoothing. We attempted a direct extension of this idea with DASM, but it didn’t give expected results. The main challenge is that we don’t have direct supervision on these maps. }
